Fuzzy temporal convolutional neural networks in P300-based Brain-computer interface for smart home interaction

The processing and classification of electroencephalographic signals (EEG) are increasingly performed using deep learning frameworks, such as convolutional neural networks (CNNs), to generate abstract features from brain data, automatically paving the way for remarkable classification prowess. However, EEG patterns exhibit high variability across time and uncertainty due to noise. It is a significant problem to be addressed in P300-based Brain Computer Interface (BCI) for smart home interaction. It operates in a non-optimal natural environment where added noise is often present. In this work, we propose a sequential unification of temporal convolutional networks (TCNs) modified to EEG signals, LSTM cells, with a fuzzy neural block (FNB), which we called EEG-TCFNet. Fuzzy components may enable a higher tolerance to noisy conditions. We applied three different architectures comparing the effect of using block FNB to classify a P300 wave to build a BCI for smart home interaction with healthy and post-stroke individuals. Our results reported a maximum classification accuracy of 98.6% and 74.3% using the proposed method of EEG-TCFNet in subject-dependent strategy and subject-independent strategy, respectively. Overall, FNB usage in all three CNN topologies outperformed those without FNB. In addition, we compared the addition of FNB to other state-of-the-art methods and obtained higher classification accuracies on account of the integration with FNB. The remarkable performance of the proposed model, EEG-TCFNet, and the general integration of fuzzy units to other classifiers would pave the way for enhanced P300-based BCIs for smart home interaction within natural settings.

==> legacy/legacy.tex <==
%%% OLD RELATED WORKS

%------------------------------------------------------------
%------------------------------------------------------------
\subsection{Convolutional Neural Networks (CNN) in BCI}
%------------------------------------------------------------
%-----------------------------------------------------------
Several techniques have been applied to EEG analysis using CCN. For instance, Ceccoti \cite{cecotti2017convolutional} applied six CNN topologies with different layer dimensions to achieve the P300 response with a 64-channel system in 16 subjects; consequently, the results indicate an average accuracy of 0.905 area under the curve (AUC) and the highest performance of 0.897 + 0.044 AUC. Similarly, in \cite{vavreka2020evaluation}, the P300 classifier using CNN models is applied in 250 subjects (138 men and 112 women), obtaining an average accuracy between $62\%$ and $64\%$ after optimization criteria improved the CNNs parameters in each test.  In \cite{cecotti20193d}, 3D and 2D CNNs classified event-related potential (ERP) to compare these architectures clearly. Among the four 3D models and two 2D models, the higher dimension model reached the result with a 0.928 + 0.05 AUC efficiency. Particular models were also studied in \cite{lawhern2018eegnet}, where  an EEGNet topology obtained an accuracy of $66.7\%$ in ERP for a P300 wave response. This model provides a low computational cost and has fewer parameters (1716) than other commonly used architectures. Recently other derivative architectures 

\subsection{Temporal Convolutional Neural Network (TCNN) in BCI}

The TCNN architecture provides specific task classification for sequential modeling \cite{bai2018empirical}. Therefore, TCNNs accomplished higher results than standard models in image processing, language, and musical data \cite{lin2020temporal}. In \cite{pandey2019tcnn}, Pandey and Wang implemented an encoder-decoder architecture with a Temporal Convolutional Module (TCM) between these codification structures; the final model is called TCNN. The TCNN proposed aims to improve real-time speech in the time domain using a different voice and noise data; therefore, the results indicate the highest accuracy of 88.10%.

Subsequently, TCNNs architectures were applied in human activity recognition (HAR). Ward et al.  \cite{ward2019dilated} proposed a Dilated TCNN with independently component layers for cognitively disabled people, resulting in an average accuracy of $92.66\%$ with one-channel accelerometer information. In BCI applications, an EEG-based spatio-temporal convolutional neural network (ESTCNN) is applied to detect driver fatigue in eight subjects. The study evaluated alert and fatigue states to train the network with undersampled trials; consequently, the model achieved the highest accuracy of $97.37\%$ compared to eight similar topologies \cite{gao2019eeg}. Moreover, in \cite{ingolfsson2020eeg}, an EEG-TCNet, a combination of an EEGNet and TCN, provided both an efficient parameter optimization and higher average classification than standard models for EEG analysis. The system processed signals of 22-channels from 15 subjects, resulting in an average accuracy of $77.35\%$. After an intra-subject optimization, the accuracy increased to $83.84\%$. 

\subsection{Long-Short Term Memory (LSTM) in BCI}

The LSTM network was applied in several BCI systems. In \cite{das2019spatio}, Das et al. proposed a sequential algorithm using a CNN for feature extraction and LSTM for task-subject pair classification. The algorithm was tested with data of 64-channels from 109 subjects in two situations: Eye Closed (EC) and Eye Open (EO). The results indicated an average accuracy of $99.95\%$ and $98\%$ for EC and EO, respectively. Additionally, in \cite{ditthapron2019universal}, an event-related potential autoencoder neural network (ERPENet) is created to compress EEG input signals simultaneously, then extract relevant features. The ERPENet classifier results in an 0.1147 + 0.0326 mean-squared error (MSE) and efficiency of $88.52 + 2.42\%$. The work in \cite{wang2020temporal} presents a BCI application with an LSTM network to extract temporal-spatial-frequency EEG characteristics; therefore, the work proposes two parallel and two serial structures, where the CNN extracts frequency characteristics, and the LSTM, temporal. Results indicate the highest precision of $85.6\%$ for the serial compact convolutional recurrent neural network (SCCRNN). 

\subsection{Fuzzy Networks}
The Fuzzy Logic implementation in neural networks has proven successful in several applications. In \cite{rovzman2020privacy}, a Big Bang - Big Crunch (BB-BC) type 2 classification system is implemented to detect facial gesture recognition, resulting in a similar accuracy compared to a Deep Neural Network (DNN).  Regarding neural networks with fuzzy systems topologies, Sharma et al. \cite{sharma2019fuzzy} presented a dimensionality reduction technique with Fuzzy Logic and reinforced it with a CNN, which improves efficiency. In consequence, the network was trained and evaluated with the MNIST database using a standard grouping (maximum-minimum) approach. The average accuracies were: an average of $88.48\%$ for the maximum group, $94.064\%$ for the medium group, and $94.4\%$ for the Fuzzy group. Additionally, in \cite{yeganejou2019interpretable}, a topology with CNNs for feature extraction attached to a Fuzzy classification system, in a derived feature space, proves the improvement of connecting a neural net and a Fuzzy system. Lastly, the work illustrated in \cite{assunccao2020intermediary} identifies the user mood based on emotion detection. The middle layer Fuzzy system was included in a CNN-based VGGVox topology, where the trained network improves the previous results in four datasets  with an average accuracy of $78.5\%$, the highest result among similar topologies without a Fuzzy layer.
